PINNferring the Hubble Function with Uncertainties

The Hubble function characterizes a given Friedmann-Robertson-Walker spacetime and can be related to the densities of the cosmological fluids and their equations of state. We show how physics-informed neural networks (PINNs) emulate this dynamical system and provide fast predictions of the luminosity distance for a given choice of densities and equations of state, as needed for the analysis of supernova data. We use this emulator to perform a model-independent and parameter-free reconstruction of the Hubble function on the basis of supernova data. As part of this study, we develop and validate an uncertainty treatment for PINNs using a heteroscedastic loss and repulsive ensembles.

==> PINNsuper/incl_settings.tex <==
% ========================================================================================
% SciPost LaTeX Template (version 2021-08)
% [https://scipost.org/SciPostPhys/authoring#manuprep]
% [https://git.scipost.org/scipost/SciPost_LaTeX_Templates_Submission]
% slightly adapted/customized by Lorenz Vogel (version 2022-01)
% Plehn Group, Institute for Theoretical Physics, Heidelberg University
% [compiler: pdfLaTeX]
% ========================================================================================

\usepackage[utf8]{inputenc} % input encodings (allow UTF-8 input)
\usepackage[T1]{fontenc} 	% selecting font encodings (use 8-bit T1 fonts)
\usepackage[english]{babel} % multilingual support (English language/hyphenation)

% note: in case the sans serif URL links look jagged/pixelated,
% this may be because you are using MiKTeX and have not yet installed "cm-super"
% solution: first, try to install the "cm-super" package via the "MiKTeX Console"
% alternative: if that doesn't work, the "lmodern" package can be used instead
%\usepackage{lmodern} 		% Latin Modern fonts

% SciPost font typeface and (sans serif or roman) URL style
\usepackage[bitstream-charter]{mathdesign}
\urlstyle{rm} %\urlstyle{sf}

\usepackage{geometry} 		% flexible and complete interface to document dimensions
%\usepackage{microtype} 	% subliminal refinements towards typographical perfection
\usepackage{amsmath} 		% math package (American Mathematical Society)
%\usepackage{amssymb} 		% math package (extended symbol collection)
%\usepackage{amsthm} 		% math package (typesetting theorems using AMS style)
\usepackage{mathtools} 		% math package (fixes various deficiencies of amsmath)
\usepackage{float} 			% floating objects such as figures and tables
\usepackage{graphicx} 		% enhanced support for graphics
\usepackage{tabularx} 		% tabulars with adjustable-width columns
\usepackage{booktabs} 		% professional-quality tables
\usepackage{color, xcolor} 	% foreground and background colour management
\usepackage{pdfpages} 		% inclusion of external multi-page PDF documents
\usepackage{extarrows} 		% extra arrows beyond those provided in amsmath
\usepackage{multirow} 		% create tabular cells spanning multiple rows
\usepackage{multicol} 		% intermix single and multiple columns
%\usepackage{caption} 		% customising captions in floating environments
%\usepackage{subcaption} 	% support for sub-captions (captions for subfigures)
%\usepackage{subfigure}
\usepackage[subrefformat=parens]{subcaption}
\usepackage{enumitem} 		% control layout of itemize, enumerate, description
%\usepackage{setspace} 		% set space between lines (single, onehalf, double)
\usepackage{xspace} 		% define commands that appear not to eat spaces
%\usepackage{ragged2e} 		% alternative versions of ragged-type commands
\usepackage{stackrel} 		% enhancement to the \stackrel command
\usepackage{tikz} 			% create PostScript and PDF graphics
\usetikzlibrary{calc}
\usepackage{braket} 		% Dirac bra-ket notation
\usepackage{bm} 			% access bold symbols in maths mode
\usepackage{tensor} 		% typeset tensors (tensor-style super- and subscripts)
\usepackage{slashed} 		% slash through characters (Feynman slash notation)
\usepackage{siunitx} % SI units package (typesetting values with units)
\usepackage{lastpage} 		% reference last page
\usepackage{cite} 			% improved citation handling
\usepackage[normalem]{ulem} % package for underlining
\usepackage{fontawesome} 	% access to web-related icons
\usepackage{tocloft} 		% control over the typography of the TOC, LOF, and LOT
\usepackage{titlesec} 		% interface to sectioning commands (various title styles)
\usepackage{doi} 			% create correct hyperlinks for DOI numbers
\usepackage{hyperref} 		% hypertext links (handel cross-referencing commands)
\usepackage[most]{tcolorbox} 					% coloured and framed text boxes
\usepackage[nameinlink, capitalize]{cleveref} 	% intelligent cross-referencing
\usepackage[nottoc, notlot, notlof]{tocbibind} 	% add references/index/contents to TOC
\usepackage[ruled, vlined]{algorithm2e} 		% floating algorithm environment
%\usepackage{dsfont}             % additional math fonts
\usepackage{makecell}
\usepackage{setspace}
\usepackage{orcidlink}

% prevent all line breaks in inline equations
\binoppenalty=10000
\relpenalty=10000

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\makeatletter
\@ifundefined{pdfoutput}{}{\DeclareGraphicsRule{*}{mps}{*}{}}
\makeatother

\makeatletter
\DeclareRobustCommand*{\bfseries}{%
   \not@math@alphabet\bfseries\mathbf
   \fontseries\bfdefault\selectfont
   \boldmath
}
\makeatother

\sisetup{
	exponent-product={\times},
	separate-uncertainty = true,
	table-align-text-pre = false,
	table-align-text-post= false,
	tight-spacing=false,
	table-align-exponent=false,
	group-digits=false,
	multi-part-units=single,
}

\hypersetup{
	colorlinks=true, 			% false: boxed links, true: colored links
	linkcolor={red!50!black}, 	% color of internal links (sections, pages, etc.)
	citecolor={blue!50!black}, 	% color of citation links (links to bibliography)
	urlcolor={blue!80!black} 	% color of URL links (external links)
} 
% more hypersetup options: 
% linktoc=none,section,page,all (defines which part in the TOC is made into a hyperlink)
% hidelinks (removing color and border)

% fix \cal and \mathcal characters look (so it's not the same as \mathscr)
\DeclareSymbolFont{usualmathcal}{OMS}{cmsy}{m}{n}
\DeclareSymbolFontAlphabet{\mathcal}{usualmathcal}

% default setup and general settings
%\sisetup{separate-uncertainty=true}
%\numberwithin{equation}{section}
%\numberwithin{figure}{section}
%\numberwithin{table}{section}

% algorithm environment settings
\renewcommand{\algorithmautorefname}{Algorithm}
\newcommand\mycommfont[1]{\textcolor{gray}{#1}}
\SetArgSty{textnormal}
\SetKwComment{Comment}{{\small\#}~}{}
\SetCommentSty{mycommfont}

% more options: leftmargin=*, topsep=2pt, partopsep=0pt, labelindent=3pt
\setitemize{itemsep=0pt, parsep=0pt} 				% adjust itemize environment
\setenumerate{itemsep=0pt, parsep=0pt} 				% adjust enumerate environment
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 	% footnote symbol
\setlength{\tabcolsep}{5pt}		% adding space between columns in a table
\setlength{\parskip}{3pt} 		% parameter that characterises the paragraph spacing
%\setlength{\parindent}{0pt} 	% parameter that characterises the paragraph indentation

% maximal number of floating environments on each page (default values)
%\setlength{\floatsep}{0pt} 			% vertical space between floating objects
%\setcounter{topnumber}{2} 				% maximum number of floats at top of page 
%\setcounter{bottomnumber}{1} 			% maximum number of floats at bottom of page 
%\setcounter{totalnumber}{3} 			% maximum number of floats on a page
%\renewcommand{\topfraction}{0.7} 		% maximum fraction of page for floats at top
%\renewcommand{\bottomfraction}{0.3} 	% maximum fraction of page for floats at bottom
%\renewcommand{\textfraction}{0.2} 		% minimum fraction of page for text

% To fix list things: 
\setitemize{itemsep=2pt,topsep=2pt,parsep=0pt,partopsep=0pt,leftmargin=*}
\setenumerate{itemsep=0pt,topsep=2pt,parsep=0pt,partopsep=0pt,labelindent=3pt,leftmargin=*}
\setlength{\tabcolsep}{2pt}

\usepackage{placeins}



==> PINNsuper/incl_shortcuts.tex <==
%-----------------------------------------------------------------------
%\marginparwidth 4.7cm
%\setlength{\hoffset}{-2.5cm}
\newcommand{\mpar}[1]{{\marginpar{\hbadness10000%
                     \sloppy\hfuzz10pt\boldmath\bf\footnotesize#1}}%
                      \typeout{marginpar: #1}\ignorespaces}
\def\mda{\mpar{\hfil$\downarrow$\hfil}\ignorespaces}
\def\mua{\mpar{\hfil$\uparrow$\hfil}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$\hfil]%
                  {\boldmath\hfil$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
%-----------------------------------------------------------------------

% --- spirou's commands --- %
\newcommand{\ltsima}{$\; \buildrel < \over \sim \;$}
\newcommand{\lsim}{\lower.5ex\hbox{\ltsima}}
\newcommand{\gtsima}{$\; \buildrel > \over \sim \;$}
\newcommand{\gsim}{\lower.5ex\hbox{\gtsima}}
%\newcommand{\bra}{\langle}
%\newcommand{\ket}{\rangle}
\newcommand{\dang}{d_\mathrm{A}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\p}{\mathrm{p}}

\newcommand{\ci}{\mathrm{i}}
\newcommand{\vecx}{\bmath{x}}
\newcommand{\geo}{\vecx(\btheta,\chip)}
\newcommand{\vecl}{\bmath{\ell}}
\newcommand{\veclp}{\bmath{\ell}^\prime}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\dlp}{(\ell-\lprime)}

\newcommand{\chip}{{\chi^\prime}}
\newcommand{\chipp}{{\chi^{\prime\prime}}}
\newcommand{\lprime}{\ell^\prime}
\newcommand{\dirac}{\delta_D}
\newcommand{\likeli}{\mathcal{L}}
\newcommand{\ham}{\mathcal{H}}

\newcommand{\ie}{i.e.\@\xspace} 		% id est (i.e.)
\newcommand{\eg}{e.g.\@\xspace} 		% exempli gratia (e.g.)
\newcommand{\vs}{vs.\@\xspace} 			% versus (vs.)
\newcommand{\etal}{et~al.\@\xspace}		% et al.
\newcommand{\eqcomma}{\;\text{,}} 		% equation comma
\newcommand{\eqperiod}{\;\text{.}} 		% equation period
\newcommand{\doublehat}[1]{\hat{\hat{#1}}}

% red, green, and blue comments
\def\tcb#1{\textcolor{blue}{#1}}
\def\tcr#1{\textcolor{red}{#1}}
\def\tcg#1{\textcolor{darkgreen}{#1}}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

% SFitter stuff
\newcommand{\sfitter}{\textsc{SFitter}\xspace}

% brackets and parentheses
\newcommand{\doublet}[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand{\ccdot}{\!\cdot\!}
\newcommand{\mueff}{\mu_{\text{eff}}}
\newcommand{\tbl}{\tan\beta}
\newcommand{\tbp}[1]{\tan^#1\beta}
\newcommand{\tb}{t_{\beta}}
\newcommand{\tbz}{t_{2\beta}}
\newcommand{\OS}{\text{OS}}
\newcommand{\cwl}{\cos\theta_W}
\newcommand{\cbl}{\cos\beta}
\newcommand{\cbp}[1]{\cos^#1\beta}
\newcommand{\DRbar}{\overline{\text{DR}}}

\newcommand{\Langle}{\bigl\langle}
\newcommand{\Rangle}{\bigr\rangle}
\newcommand{\XLangle}{\Bigl\langle}
\newcommand{\XRangle}{\Bigr\rangle}
\newcommand{\XXLangle}{\biggl\langle}
\newcommand{\XXRangle}{\biggr\rangle}
\newcommand{\XXXLangle}{\Biggl\langle}
\newcommand{\XXXRangle}{\Biggr\rangle}
\newcommand{\Lbrack}{\bigl\lbrack}
\newcommand{\Rbrack}{\bigr\rbrack}
\newcommand{\XLbrack}{\Bigl\lbrack}
\newcommand{\XRbrack}{\Bigr\rbrack}
\newcommand{\XXLbrack}{\biggl\lbrack}
\newcommand{\XXRbrack}{\biggr\rbrack}
\newcommand{\Lbrace}{\bigl\lbrace}
\newcommand{\Rbrace}{\bigr\rbrace}
\newcommand{\XLbrace}{\Bigl\lbrace}
\newcommand{\XRbrace}{\Bigr\rbrace}
\newcommand{\XXLbrace}{\biggl\lbrace}
\newcommand{\XXRbrace}{\biggr\rbrace}
\newcommand{\braces}[1]{\lbrace#1\rbrace}
\newcommand{\bigbraces}[1]{\bigl\lbrace#1\bigr\rbrace}
\newcommand{\bigbrackets}[1]{\bigl\lbrack#1\bigr\rbrack}

\newcommand{\qqquad}{\qquad\quad}
\newcommand{\qqqquad}{\qquad\qquad}

% general math definitions
\def\D{\mathrm{d}}
%\newcommand{\diff}{\mathop{}\!\mathrm{d}} 	% differential
\newcommand{\diff}{\mathrm{d}} 				% differential
\newcommand{\del}{\partial} 				% partiallderivative
\newcommand{\abs}[1]{\lvert#1\rvert} 		% absolute value (single vertical lines)
\newcommand{\norm}[1]{\lVert#1\rVert} 		% norm (double vertical lines)
\newcommand{\Z}{\mathbb{Z}} 				% integers
\newcommand{\Q}{\mathbb{Q}} 				% rational numbers
\newcommand{\R}{\mathbb{R}} 				% real numbers
\newcommand{\var}{\operatorname{Var}} 		% variance
\newcommand{\sign}{\operatorname{sign}} 	% sign
\newcommand{\tr}{\operatorname{Tr}}			% trace
\newcommand{\order}{\mathcal{O}} 			% order
\newcommand{\imag}{\mathrm{i}} 				% imaginary unit
\newcommand{\euler}{\mathrm{e}} 			% Euler's number
\newcommand{\iid}{\text{i.i.d.}} 			% independent and identically distributed
\newcommand{\crange}[2]{#1,\ldots,#2}		% range with comma
\newcommand{\range}[2]{#1\:\!\ldots\:\!#2}	% range without comma
\newcommand{\really}{\stackrel{!}{=}}
\newcommand{\mean}[1]{\langle#1\rangle}
\newcommand{\one}{\mathbb{1}}

% particle physics and machine learning definitions
\newcommand{\similarity}{\operatorname{sim}}
\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\sigmoid}{\operatorname{sigmoid}}
\newcommand{\relu}{\operatorname{ReLU}}
\newcommand{\leakyrelu}{\operatorname{LeakyReLU}}
\newcommand{\attention}{\operatorname{Attention}}
\newcommand{\multihead}{\operatorname{MultiHead}}
\newcommand{\concat}{\operatorname{Concat}}
\newcommand{\head}{\operatorname{head}}

\newcommand{\normal}{\mathcal{N}}
\newcommand{\lag}{\mathscr{L}}
\newcommand{\ope}{\mathcal{O}}
\newcommand{\obs}{\mathcal{O}}
\newcommand{\uniform}{\mathcal{U}}
\newcommand{\sqrts}{\sqrt{s}} 		% center-of-mass energy
\newcommand{\loss}{\mathcal{L}} 	% loss value
\newcommand{\like}{\mathcal{L}} 	% loss value
\newcommand{\dth}{\Delta_\text{th/sys}}
\newcommand{\dst}{\Delta_\text{stat}}
\newcommand{\dsy}{\Delta_\text{syst}}

\newcommand{\batch}{\mathrm{batch}}
\newcommand{\nbatch}{N_\text{batch}}
\newcommand{\nc}{n_{C}} % number of constituents
\newcommand{\kl}{\operatorname{KL}}

\newcommand{\vpd}{\vec{p}_\text{data}}
\newcommand{\vpmd}{\vec{p}_\text{model}}
\newcommand{\pdj}[1]{p_{\text{data},#1}}
\newcommand{\pmdj}[1]{p_{\text{model},#1}}
\newcommand{\pl}{p_\text{latent}}
\newcommand{\pd}{p_\text{data}}
\newcommand{\pmd}{p_\text{model}}
\newcommand{\pfw}{p}
\newcommand{\pbw}{p_\theta}

% particle-flow objets
\newcommand{\npf}{n_\text{PF}}
\newcommand{\wpf}{w_\text{PF}}
\newcommand{\ptd}{p_\text{T}D}
\newcommand{\xmax}{x_{\mathrm{max}}}
\newcommand{\pid}{\mathrm{PID}}

\newcommand{\etaphi}{$\eta$--$\phi$\xspace} % eta-phi plane
\newcommand{\auc}{\mathrm{AUC}} % area under the ROC curve
\newcommand{\es}{\epsilon_{s}} 	% signal efficiency (true-positive rate)
\newcommand{\eb}{\epsilon_{b}} 	% background mistag rate (false-positive rate)
\newcommand{\imtafe}{\epsilon_{b}^{-1}(\epsilon_{s}\!=\!0.5)}
\newcommand{\imtafeqg}[1]{\epsilon_{g}^{-1}(\epsilon_{q}\!=\!#1)}
\newcommand{\sklearn}{\texttt{scikit-learn}\xspace}
\newcommand{\pytorch}{\textsc{PyTorch}\xspace}
\newcommand{\tensorflow}{\textsc{TensorFlow}\xspace}
\newcommand{\adam}{\textsc{Adam}\xspace}
\newcommand{\adamw}{\textsc{AdamW}\xspace}
\newcommand{\energyflow}{\textsc{EnergyFlow}\xspace}
\newcommand{\fastjet}{\textsc{FastJet}\xspace}
\newcommand{\pythia}{\textsc{Pythia}\xspace}
\newcommand{\herwig}{\textsc{Herwig}\xspace}
\newcommand{\delphes}{\textsc{Delphes}\xspace}
\newcommand{\rivet}{\textsc{Rivet}\xspace}
\newcommand{\python}{\textsc{Python}\xspace}
\newcommand{\numpy}{\textsc{NumPy}\xspace}
\newcommand{\vegas}{\textsc{Vegas}\xspace}
\newcommand{\madgraph}{\textsc{Madgraph}\xspace}
\newcommand{\sherpa}{\textsc{Sherpa}\xspace}
\newcommand{\keras}{\textsc{Keras}\xspace}

\newcommand{\py}{\textsc{Py}}
\newcommand{\he}{\textsc{He}}
\newcommand{\sh}{\textsc{Sh}}
\newcommand{\mup}{\mu_{\mathrm{pred}}}
\newcommand{\sip}{\sigma_{\mathrm{pred}}}

\newcommand{\efp}{\mathrm{EFP}} 		% energy flow polynomials
\newcommand{\ttbar}{t\bar{t}} 			% top-antitop pair
\newcommand{\electron}{\mathrm{e}^{-}} 	% electron
\newcommand{\positron}{\mathrm{e}^{+}} 	% positron

% hyperlink references
\newcommand{\urlx}[1]{\href{#1}{#1}}
\newcommand{\DOI}[2]{\href{http://dx.doi.org/#2}{#1}}
%\newcommand{\arXiv}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1}}
\newcommand{\arXiv}[2][]{%
	\ifthenelse{\equal{#1}{}}%
	{\href{http://arxiv.org/abs/#2}{arXiv:#2}}%
	{\href{http://arxiv.org/abs/#2}{arXiv:#2~[#1]}}}

% units of measure
\newcommand{\cmu}{\text{cm}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ab}{\text{ab}}
\newcommand{\pb}{\text{pb}}
\newcommand{\br}{\text{BR}}
\newcommand{\ifb}{\ensuremath{\text{fb}^{-1}} }
\newcommand{\iab}{\ensuremath{\text{ab}^{-1}} }
\newcommand{\ipb}{\text{pb}^{-1}}

% really great macro by Chris Lester
\def\slashchar#1{\setbox0=\hbox{$#1$}           % set a box for #1
   \dimen0=\wd0                                 % and get its size
   \setbox1=\hbox{/} \dimen1=\wd1               % get size of /
   \ifdim\dimen0>\dimen1                        % #1 is bigger
      \rlap{\hbox to \dimen0{\hfil/\hfil}}      % so center / in box
      #1                                        % and print #1
   \else                                        % / is bigger
      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}   % so center #1
      /                                         % and print /
   \fi}
\newcommand{\dslash}{\slashchar{\partial}}
\newcommand{\Dslash}{\slashchar{D}}
\newcommand{\met}{\slashchar{E}_T}

%\DeclareMathOperator{\tr}{Tr}

% for transformation matrix A
\newcommand{\tikznode}[2]{%
\ifmmode%
\tikz[remember picture,baseline=(#1.base),inner sep=0pt] \node (#1) {$#2$};%
\else
\tikz[remember picture,baseline=(#1.base),inner sep=0pt] \node (#1) {#2};%
\fi}

% nice looking particle names and masses
\def\mathswitchr#1{\relax\ifmmode{\text{#1}}\else$\text{#1}$\xspace\fi}
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\xspace\fi}
\newcommand{\Pf}{\mathswitch  f}
\newcommand{\Pfbar}{\mathswitch{\bar f}}
\newcommand{\Pq}{\mathswitch q}
\newcommand{\Pqbar}{\mathswitch{\bar q}}
\newcommand{\PW}{\mathswitchr W}
\newcommand{\PWp}{\mathswitchr {W^+}}
\newcommand{\PWm}{\mathswitchr {W^-}}
\newcommand{\PWpm}{\mathswitchr {W^\pm}}
\newcommand{\PZ}{\mathswitchr Z}
\newcommand{\PZp}{\mathswitchr {Z'}}
\newcommand{\Pg}{\mathswitchr g}
\newcommand{\PH}{\mathswitchr H}
\newcommand{\Pe}{\mathswitchr e}
\newcommand{\Pne}{\mathswitch \nu_{\text{e}}}
\newcommand{\Pep}{\mathswitchr {e^+}}
\newcommand{\Pem}{\mathswitchr {e^-}}
\newcommand{\Pmup}{\mu^+}
\newcommand{\Pgngm}{\nu_\mu}
\newcommand{\Pp}{\mathswitchr p}
\newcommand{\Pd}{\mathswitchr d}
\newcommand{\Pu}{\mathswitchr u}
\newcommand{\Ps}{\mathswitchr s}
\newcommand{\Pc}{\mathswitchr c}
\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pt}{\mathswitchr t}
\newcommand{\Pj}{\mathswitchr j}
\newcommand{\Ptbar}{\mathswitchr{\bar t}}
\newcommand{\jet}{\text{jet}}
\newcommand{\jets}{\text{jets}}
\newcommand{\Pl}{\ell}
\newcommand{\Mf}{\mathswitch {m_\Pf}}
\newcommand{\Ml}{\mathswitch {m_\Pl}}
\newcommand{\Mq}{\mathswitch {m_\Pq}}
\newcommand{\MV}{\mathswitch {M_\PV}}
\newcommand{\MW}{\mathswitch {M_\PW}}
\newcommand{\MA}{\mathswitch {\lambda}}
\newcommand{\MZ}{\mathswitch {M_\PZ}}
\newcommand{\MZp}{\mathswitch {M_\PZp}}
\newcommand{\MH}{\mathswitch {M_\PH}}
\newcommand{\Me}{\mathswitch {m_\Pe}}
\newcommand{\Mmy}{\mathswitch {m_\mu}}
\newcommand{\Mta}{\mathswitch {m_\tau}}
\newcommand{\Md}{\mathswitch {m_\Pd}}
\newcommand{\Mu}{\mathswitch {m_\Pu}}
\newcommand{\Ms}{\mathswitch {m_\Ps}}
\newcommand{\Mc}{\mathswitch {m_\Pc}}
\newcommand{\Mb}{\mathswitch {m_\Pb}}
\newcommand{\Mt}{\mathswitch {m_\Pt}}




